SCHENO: Measuring Schema vs. Noise in Graphs

Real-world data is typically a noisy manifestation of a core pattern (schema), and the purpose of data mining algorithms is to uncover that pattern, thereby splitting (i.e. decomposing) the data into schema and noise. We introduce SCHENO, a principled evaluation metric for the goodness of a schema-noise decomposition of a graph. SCHENO captures how schematic the schema is, how noisy the noise is, and how well the combination of the two represent the original graph data. We visually demonstrate what this metric prioritizes in small graphs, then show that if SCHENO is used as the fitness function for a simple optimization strategy, we can uncover a wide variety of patterns. Finally, we evaluate several well-known graph mining algorithms with this metric; we find that although they produce patterns, those patterns are not always the best representation of the input data.

==> figures/sst_preamble.tex <==
\usepackage{tikz,amsmath, amssymb,bm,color}
\usepackage{multirow} %, multicol}
\usepackage{colortbl}
\usepackage{enumitem}
\usetikzlibrary{shapes,arrows, arrows.meta}
% Satyaki, I (Justus) removed `ducks` so I can compile locally. Please include only if you need it.
\usetikzlibrary{backgrounds,calc,arrows,decorations.markings, shapes,shapes.arrows,optics,patterns,hobby, fit, positioning, automata}
% needed for BB
% Satyaki, I (Justus) commented out this so that I can latex compile it on my machine. Please use only if you need it.
\usetikzlibrary{calc}
\usepackage{pgfplots}
\usetikzlibrary{pgfplots.groupplots}
% \selectcolormodel{cmyk}
\usepgfplotslibrary{dateplot,fillbetween}
\pgfplotsset{compat=newest}

% Allows for better url line breaks:
\Urlmuskip = 0mu plus 1mu

% some LaTeX code
\tikzstyle{textnode} = [rectangle, inner sep=0pt,outer sep=0,execute at begin node={\strut}, font=\small]  
\tikzstyle{opencircle} = [circle, thick, draw=black!80, minimum width=10, fill=black!5, inner sep=1.5, text=black]
\tikzstyle{faintopencircle} = [circle,minimum width=10, draw=black!40, fill=black!05, inner sep=1.5, text=black!40]
\tikzstyle{itxset} = [rounded corners=3pt, draw, minimum height=14pt, inner sep=0]
\tikzstyle{itxsetfocus} = [itxset, ultra thick]
\tikzstyle{internalnode} = [textnode,circle, draw=black, very thick, fill, text=black]
\tikzstyle{externalnode} = [textnode, circle, draw, thick]
\tikzstyle{nonterminal} = [textnode,draw,inner xsep=1.5]
\tikzstyle{graphletnode} = [circle, draw, fill, minimum size=1.0mm,inner sep=0pt,outer sep=0pt, fill=black]
\tikzstyle{splitnode} = [circle, draw, fill=black, minimum size=2.2mm,inner sep=0pt,outer sep=0pt]
\tikzset{ghost/.style={color=gray!50}}
\tikzstyle{faintnonterminal} = [draw=black!40, inner sep=1.5, text=black!40]
\tikzstyle{faintedge} = [very thin, color=black!50]
\tikzstyle{enode-hrg} = [circle, draw, fill=black, text=white, minimum size=4mm, inner sep=0.25pt, outer sep=1.5pt]  % external node for HRGs
\tikzstyle{hyperedge} = [draw, inner xsep=0.5, fill=gray!5, diamond, minimum size=0.5mm, outer sep=0.5pt]  % non-terminal node 


%% tikz shapes
\tikzstyle{textnode} = [rectangle, inner sep=0pt,outer sep=0,execute at begin node={\strut}, font=\small]  % text nodes 

\tikzstyle{bnode} = [circle, draw, fill=NDblue, minimum size=2mm, text=white, outer sep=1pt]  % boundary nodes

\tikzstyle{enode} = [circle, draw=white, thick, inner sep=1.5pt, fill=gray!20, outer sep=2pt, text=black]  % external nodes

\tikzstyle{inode} = [circle, thick, minimum size=5pt, draw=black, fill=gray!10!white, inner sep=0pt, outer sep=1.5pt]  % internal nodes 

\tikzstyle{nt} = [draw=pastelred, very thick, rectangle, inner xsep=1.5, fill=gray!5, minimum width=3mm, minimum height=5mm, outer sep=2pt, text=black, font=\large]  % non-terminal node 

\tikzstyle{tnode} = [minimum size=5mm, font=\large]  % terminal node

\tikzstyle{hnode} = [enode, very thick, draw=NDgold]  % highlighted nodes

\tikzstyle{hidden} = [draw=none, rectangle]

\tikzstyle{edge} = [thick, draw=black]  % edge style

\tikzstyle{iedge} = [edge, very thick, draw=gray]   % internal edge

\tikzstyle{bedge} = [edge, draw=NDgreen]  % boundary edge

\tikzstyle{deledge} = [edge, draw=red, dotted]  % boundary edge

\tikzstyle{faded} = [opacity=0.40, text opacity=0.40]

\tikzstyle{newnode} = [circle, thick, minimum size=2mm, outer sep=1.5pt, draw=blue,fill=cyan!50]  % internal nodes 

\tikzstyle{Arrow} = [line width=0.5mm, draw=NDgold!80, -{Triangle[length=1.55mm,width=0.95mm]}, scale=0.75, transform shape]

\tikzstyle{hedge} = [edge, ->, very thick, draw=gray!80]

\tikzstyle{nedge} = [hedge, draw=cyan!80]

\tikzstyle{redge} = [hedge, draw=red!60]

% \tikzset{diredge/.style={->, >= latex', thick}}
\tikzstyle{diredge} = [->, >={latex'[length=1mm]}, thick]
\tikzstyle{boundedge} = [diredge, draw=NDgold]  % boundary edge

\tikzset{newedge/.style = {->,> = latex', very thick}}

\tikzstyle{uedge} = [thick, shorten >=1pt, auto,]  % edge style

\tikzstyle{highlight} = [very thick, preaction={fill=gray!50}, pattern=north east lines]

\tikzstyle{shrink} = [scale=0.5, transform shape]

\tikzstyle{treenode} = [enode, shrink]

\tikzstyle{tedge} = [->, >=latex, draw=gray, thin]

\tikzstyle{tedge2} = [-{Latex[length=1mm]}, draw=gray, thin]

\tikzstyle{blob} = [ellipse, draw=black, dashed, minimum height=40pt, minimum width=37.5, outer sep=1.5pt]
\tikzstyle{dottededge} = [edge, dashed]

\tikzstyle{sourceinode} = [inode, fill=gray!80]
\tikzstyle{targetinode} = [inode, fill=black!80]


\tikzstyle{newestdiredge} = [diredge, draw=blue!50!cyan, fill=blue!50!cyan]
\tikzstyle{newdiredge} = [diredge, draw=blue!80!white, fill=blue]
\tikzstyle{olddiredge} = [diredge, draw=gray, fill=gray]
\tikzstyle{neverdiredge} = [diredge, draw=cyan, fill=cyan]

\tikzstyle{t0} = [line width=1pt]
\tikzstyle{t1} = [line width=1.5pt]
\tikzstyle{t2} = [line width=2pt]
\tikzstyle{t3} = [line width=2.5pt]

%% PGFPLOTS stuff 
\usepackage{pgfplots}
\usetikzlibrary{pgfplots.groupplots}
\selectcolormodel{cmyk}

\def\rot#1{\rotatebox{90}{#1}}
% argument #1: any options
\newenvironment{customlegend}[1][]{%
    \begingroup
    % inits/clears the lists (which might be populated from previous
    % axes):
    \csname pgfplots@init@cleared@structures\endcsname
    \pgfplotsset{#1}%
}{%
    % draws the legend:
    \csname pgfplots@createlegend\endcsname
    \endgroup
}%

\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}

\pgfplotsset{
    jitter/.style={
        y filter/.code={\pgfmathparse{\pgfmathresult+rnd*#1}}
    },
    jitter/.default=0.05
}
\pgfplotsset{every tick label/.append style={font=\scriptsize}}
\pgfplotsset{compat=newest}
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}   %% some additional layers for demo
%%one bar symbol in pgfplot legend

\tikzstyle{globaloptions} = [] %[fill opacity=0.75]%, draw opacity=0.75, fill opacity=0.75]
\tikzstyle{sst} = [draw=blue, fill=blue!60, globaloptions]  
\tikzstyle{sst3} = [draw=cyan, fill=cyan!60, globaloptions]  

\tikzstyle{gcnae} = [draw=red, fill=red!60, globaloptions]  
\tikzstyle{gcnvae} = [draw=red!50, fill=red!30, globaloptions]

\tikzstyle{comm} = [draw=lime, fill=lime!60, globaloptions]
\tikzstyle{random} = [draw=black, fill=black!60, globaloptions]

\tikzstyle{linearae} = [draw=green!40!black, fill=green!70!black]  % hrg
\tikzstyle{linearvae} = [draw=green!70!black, fill=green!50!white]  % hrg

\tikzstyle{gravityae} = [draw=pink, fill=pink!50!red, globaloptions]  
\tikzstyle{gravityvae} = [draw=pink!80, fill=pink!90!red, globaloptions]

